Approximate Cross-Validation for Structured Models

Many modern data analyses benefit from explicitly modeling dependence structure in data -- such as measurements across time or space, ordered words in a sentence, or genes in a genome. A gold standard evaluation technique is structured cross-validation (CV), which leaves out some data subset (such as data within a time interval or data in a geographic region) in each fold. But CV here can be prohibitively slow due to the need to re-run already-expensive learning algorithms many times. Previous work has shown approximate cross-validation (ACV) methods provide a fast and provably accurate alternative in the setting of empirical risk minimization. But this existing ACV work is restricted to simpler models by the assumptions that (i) data across CV folds are independent and (ii) an exact initial model fit is available. In structured data analyses, both these assumptions are often untrue. In the present work, we address (i) by extending ACV to CV schemes with dependence structure between the folds. To address (ii), we verify -- both theoretically and empirically -- that ACV quality deteriorates smoothly with noise in the initial fit. We demonstrate the accuracy and computational benefits of our proposed methods on a diverse set of real-world applications.

==> app_lfo_equivalence_chain.tex <==
\section{Proof of \cref{prop:chain_equivalence}}

Recall that for a chain structured graph, we can write:
$$
	p(x,z) = p(x \mid z) p(z_1) \prod_{t=2}^T p(z_t \mid z_{t-1}).
$$
Let $\mathbf{o} = \{ 1, \dots, T'\}$ for some $T' < T$; that is, we are interested in dropping out time steps $T', \dots, T$. For weighting scheme (A) (\cref{eq:mrf_cv_data_A}), we drop out only the observations, obtaining:
%
$$ 
p_A(x,z ; w_{\mathbf{o}}) = \left( \prod_{t=1}^{T'-1} p(x_t \mid z_t) \right) p(z_1) \prod_{t=2}^T p(z_t \mid z_{t-1}).
$$
%
When we sum out all $z$ to compute the marginal $p_A (x ; w_{\mathbf{o}})$, we can first sum over $z_T$. As $\sum_{z_T} p(z_T \mid z_{T-1}) = 1$ for any value of $z_{T-1}$, we obtain:
%
$$
	p_A(x; w_\mathbf{o}) = \sum_{z_1, \dots, z_{T'-1}} \left( \prod_{t=1}^{T'-1} p(x_t \mid z_t) \right) p(z_1) \prod_{t=2}^{T'-1} p(z_t \mid z_{t-1}),
$$
%
which is exactly the formula for $p_B(x ; w_\mathbf{o})$, the marginal likelihood from following weighting scheme (B) (\cref{eq:mrf_cv_data_B}), in which we drop out both the $x_t$ and $z_t$ for $t \not\in \mathbf{o}$.

==> app_weighted_marg.tex <==
\section{Weighted marginalization for chain-structured graphs}
\label{app:chain_structured_weighted_marg}

\begin{algorithm}
\caption{\textsc{WeightedMarg} for chain-structured graphs}
\label{alg:weighted_marg_chain}
\begin{algorithmic}[1] 
\REQUIRE $\param, \xseqone, \wseqone $\\
\STATE Set $\alpha_{1k} = \exp\big[ w_1 \psi_1 (z_1 = k, x_1 ; \param) \big]$ for $k = 1, \dots, K$
\FOR{$t = 2, \dots, T$}
	\STATE Compute $\alpha_{tk}$ via \cref{eq:weighted_alpha_recursion} for $k = 1, \dots, K$.
\ENDFOR 
\RETURN $\sum_{k=1}^K \alpha_{Tk}$
\end{algorithmic}
\end{algorithm}


Here, we derive a dynamic programming implementation of \textsc{WeightedMarg}  from \cref{alg:main_algorithm} in the case of a chain-structured MRF (e.g., a HMM); we summarize this algorithm in \cref{alg:weighted_marg_chain} Such a chain-structured graph has a weighted likelihood of the form:
%
$$
	p(x, z ; \param, w) = \exp \left[ Z(\param) + \sum_{t=1}^T w_t \psi_t(z_t, x_t) + \sum_{t=2}^T w_{t-1} w_t \phi_{t-1,t}(z_{t-1}, z_t) \right].
$$
We need to implement the function:
$$
	p(x ; \param, w) = \sum_{z_T} \cdots \sum_{z_1}  p(x, z ; \param, w).
$$
To do so, we can essentially reproduce a weighted version of the forward algorithm \citep{rabiner89} by defining:
$$ 
	\alpha_{tk} := \sum_{\substack{z_1, \dots, z_{t-1} \\ z_t = k}} \exp\left[ \sum_{s=1}^t w_s \psi_s(z_s, x_s) + \sum_{s=1}^t w_{s-1} w_s \phi_{s-1, s}(z_{s-1}, z_s) \right].
$$
Notice, then, that our desired function is $\sum_k \alpha_{Tk}$. We can compute these $\alpha_{tk}$ recursively by:
\begin{equation}
	\alpha_{t+1,k} = \sum_{\ell = 1}^K \alpha_{t\ell} \exp\bigg[ w_{t+1} \psi_{t+1} (z_{t+1} = k, x_{t+1}) + w_t w_{t+1} \phi_{t, t+1}(z_t = \ell, z_{t+1} = k) \bigg],
\label{eq:weighted_alpha_recursion}
\end{equation}
with the base case $\alpha_{1k} = \exp\big[ w_1 \psi_1 (z_1 = k, x_1) \big]$. Supposing that the computation of each potential is upper bounded by some constant $C$, the computation of each $\alpha_{tk}$ runs in $O(KC)$, for a total runtime of $O(TK^2C)$.

==> priors.tex <==
We will further place priors over the parameters,
\begin{equation}
    p(\pi_k \mid \alpha) = \text{Dir}(\alpha) \propto \prod_{j=1}^K \pi_{kj}^{\alpha_j}; \forall k
\end{equation}
The prior on $\phi$ is sometimes chosen to be conjugate to the emission/observation/likelihood model $p(x_{nt} \mid z_{nt}, \phi)$ for computational convenience. Assuming a Gaussian (with unknown mean and unknown covariance) emission model, we can place a Normal Wishart prior,
\begin{equation}
\begin{split}
    \mu_{k} \mid \mu_0, \kappa, \Lambda_k &\sim \mathcal{N}(\mu_0, (\kappa\Lambda_k)^{-1}) \\
    \Lambda_{k} \mid S, \nu &\sim \text{Wishart}(\nu, S) \\
    x_{nt} \mid \{z_{nt}=k\}, \phi &\sim \mathcal{N}(x_{nt} \mid \mu_{k}, \Lambda_{k}^{-1}).
\end{split}
\end{equation}   
Here, $\phi_k = \{\mu_k, \Lambda_k \}$ and denote by $\rho = \{\mu_0, \kappa, \nu, S \}$ the set of hyper-parameters governing the prior on $\phi_k$. 

The model is completely described by the following joint distribution, 
\begin{equation}
\begin{split}
    p(x_n, &z_n, \{\pi_k\}_{k=0}^K, \phi) = p(\pi_0\mid \alpha)\prod_{k=1}^K p(\phi_k \mid \rho)p(\pi_k\mid \alpha)\\
    &p(z_{n1} \mid \pi_0)\prod_{t=2}^{T_n}p(z_{nt}\mid z_{nt-1}, \pi) \prod_{t=1}^{T_n} p(x_{nt}\mid z_{nt}, \phi).
    \end{split}
\end{equation}

Given observed $x_n$ (typically for $n = 1, \ldots, N$) and the hyper-parameters $\rho$ and $\alpha$ our goal is to infer the unknown quantities, i.e., we are interested in the posterior distribution,
$p(z_n, \phi, \pi, \pi_0 \mid x_n, \alpha, \rho)$
